Learning against Non-credible Auctions

The standard framework of online bidding algorithm design assumes that the seller commits himself to faithfully implementing the rules of the adopted auction. However, the seller may attempt to cheat in execution to increase his revenue if the auction belongs to the class of non-credible auctions. For example, in a second-price auction, the seller could create a fake bid between the highest bid and the second highest bid. This paper focuses on one such case of online bidding in repeated second-price auctions. At each time $t$, the winner with bid $b_t$ is charged not the highest competing bid $d_t$ but a manipulated price $p_t = \alpha_0 d_t + (1-\alpha_0) b_t$, where the parameter $\alpha_0 \in [0, 1]$ in essence measures the seller's credibility. Unlike classic repeated-auction settings where the bidder has access to samples $(d_s)_{s=1}^{t-1}$, she can only receive mixed signals of $(b_s)_{s=1}^{t-1}$, $(d_s)_{s=1}^{t-1}$ and $\alpha_0$ in this problem. The task for the bidder is to learn not only the bid distributions of her competitors but also the seller's credibility. We establish regret lower bounds in various information models and provide corresponding online bidding algorithms that can achieve near-optimal performance. Specifically, we consider three cases of prior information based on whether the credibility $\alpha_0$ and the distribution of the highest competing bids are known. Our goal is to characterize the landscape of online bidding in non-credible auctions and understand the impact of the seller's credibility on online bidding algorithm design under different information structures.

==> sections/app_unknown_alpha_unknown_G_new.tex <==
\section{Missing Proofs of \Cref{sec: unknown alpha unknown G}}
\label{app: unknown alpha unknown G}

\begin{proof}[Proof of \Cref{thm: unknown alpha unknown G full}]
Let $e_m$ be the $m$-th standard basis vector. According to standard analysis of exponential weight (see for example~\citep[Lemma~14]{wei2020taking}), we have for any $m_0 \in [M]$:
    \begin{align*}
        \left<q_t-e_{m_0}, \hat{\ell}_t\right> &\leq \frac{1}{\eta} D(e_{m_0}, q_t) - \frac{1}{\eta} D(e_{m_0}, q_{t+1}) + \frac{\eta}{2}\sum_{m\in [M]}q_{t,m}\hat{\ell}_{t,m}^2,
    \end{align*}
    where $D(u,v)=\sum_{m\in [M]} u_m\log\frac{u_m}{v_m}$ is the KL divergence between $u$ and $v$. Taking summation over $t\in [T]$, we have:
    \begin{align}
        \sum_{t=1}^T\left<q_t-e_{m_0}, \hat{\ell}_t\right> &\leq \frac{D(e_{m_0}, q_1)}{\eta} + \frac{\eta}{2}\sum_{t=1}^T\sum_{m\in [M]}q_{t,m}\hat{\ell}_{t,m}^2 \nonumber \\
        &= \frac{D(e_{m_0}, q_1)}{\eta} + \frac{\eta}{2}\sum_{t=1}^T\sum_{k\in [K]}\sum_{m\in [M]}\bbI\left\{b_{t, \alpha^m}=b^k\right\}  q_{t,m}\hat{\ell}_{t,m}^2 \nonumber \\
        &= \frac{D(e_{m_0}, q_1)}{\eta} + \frac{\eta}{2}\sum_{t=1}^T\sum_{k\in[K]}\sum_{m\in [M]} 
        \bbI\left\{b_{t, \alpha^m}=b^k\right\}
        \frac{q_{t,m}\bbI\{b_{t, \alpha^m} = b_t\}}{P_t(b_{t})^2}\left(1-r_t\right)^2 \nonumber \\
        &\leq \frac{D(e_{m_0}, q_1)}{\eta} + \frac{\eta}{2}\sum_{t=1}^T\sum_{k\in[K]}\sum_{m \in [M]}
        \bbI\left\{b_t=b^k\right\}
        \frac{q_{t,m}\bbI\{b_{t, \alpha^m} = b_t\}}{P_t(b_{t})^2} \nonumber \\
        &= \frac{D(e_{m_0}, q_1)}{\eta} + \frac{\eta}{2}\sum_{t=1}^T\sum_{k\in[K]}\frac{\bbI\{b_{t, \alpha_t}=b^k\}}{P_t(b^k)}. \label{eqn: exp main}
    \end{align}
    where the second inequality is because $(1-r_t) \in [0, 1]$ and the last equality is because $P_t(b_{t}) = \sum_{m\in [M]} q_{t, m}\bbI[b_{t, \alpha^m} = b_t]$. For the right hand side, we have
    \begin{align*}
        \bbE\left[\frac{\bbI\{b_{t, \alpha_t}=b^k\}}{P_t(b^k)}\right] = 1.
    \end{align*}
    Let $r_{t, \alpha^m}$ be the instantaneous reward if we follow the suggestion of the $m$-th predictor in round $t$. If $b_{t, \alpha^m}=b_t$, we have $r_{t, \alpha^m} = r_t$ and thus
    \begin{align*}
        \bbE_{\alpha_t\sim q_t}\left[\hat{\ell}_{t,m}\right] 
        = \bbE\left[\frac{\bbI\{b_{t, \alpha^m}=b_{t}\}}{P_t(b_t)}\left(1-r_t\right)\right] = \bbE\left[\frac{\bbI\{b_{t, \alpha^m}=b_{t, \alpha_t}\}}{P_t(b_{t, \alpha_t})}\left(1-r_{t, \alpha^m}\right)\right] = 1 - r_{t, \alpha^m},
    \end{align*}
    
    Therefore, taking expectation over both sides of inequality \eqref{eqn: exp main}, we obtain
    \begin{align}
        \bbE \left[\sum_{t=1}^{T} r_{t, \alpha^m_0} - \sum_{t=1}^{T} r_{t}\right] \leq \frac{D(e_{m_0},q_1)}{\eta} + \frac{\eta}{2}TK.
    \end{align}
    Picking $f_0 = f^*$, which is in the class $\calF$ by, the left-hand side above becomes exactly the expected regret $\bbE\left[\right]$.
    Finally, since $q_1$ is a uniform distribution over $\calF$, we know that $D(e_{f^*},q_1)=\log|\calF|$, and picking $\eta=\sqrt{\frac{\log|\calF|}{\sum_{t=1}^TN_t}}$ then leads to the claimed regret bound.


\end{proof}

\begin{proof}[Proof of \Cref{lem: estimate G}]
We have
\begin{align*}
    \hat{G}_t(x; \alpha) = \frac{1}{t-1} \sum_{s=1}^{t-1} \bbI \{\hat{d}_s(\alpha) \leq x\} = \frac{1}{t-1} \sum_{s=1}^{t-1} \mathbb{I}\left\{d_s \leq x + \frac{\alpha - \alpha_0}{\alpha_0}(x - b_s)\right\}.
\end{align*}
We aim to give a uniform convergence bound for $|\hat{G}_t(x) - G(x)|$. The main challenge is that we cannot directly apply DKW inequality, since $b_s$ depends on the highest competing bids in previous rounds. To handle this challenge, we bound the lower bound and upper bound of $\hat{G}_t(x; \alpha)$ separately. Since $|\alpha - \alpha_0| \leq \calK_s$, we have
\begin{align*}
    \frac{1}{T_s} \sum_{s=1}^{t-1} \bbI\{d_t \leq x - \calK_s /\alpha_0\} \leq \hat{G}_t(x; \alpha) \leq \frac{1}{t-1} \sum_{s=1}^{t-1} \bbI\{d_t \leq x + \calK_s /\alpha_0\} 
\end{align*}
Then by DKW inequality, the upper bound uniformly converges to $G(d + \calK_s /\alpha_0)$ and the lower bound uniformly converges to $G(d - \calK_s /\alpha_0)$. By the Lipschitz condition of $G$ in \Cref{asm: unknown alpha unknown G 2}, we have $\forall x \in [0, 1]$, 
\begin{align*}
    |\hat{G}_t(x) - G(x)| \leq \sqrt{\frac{\log(4/\delta)}{2(t-1)}} + B_2\calK_s /\alpha_0
\end{align*}
holds with probability at least $1 - \delta$.
\end{proof}

==> sections/unknown_alpha_unknown_G_new.tex <==
\section{Learning with Unknown $\alpha$ and Unknown $G$}
\label{sec: unknown alpha unknown G}

\paragraph{Bandit feedback.} For the last scenario with both $\alpha$ and $G$ unknown, we first consider bandit feedback. Although the seller's credibility is unknown, this case still satisfies the cross-learning property over values, i.e., \Cref{eqn: infer r_t'} holds. Thus, \Cref{algo: known alpha unknown G fpa}, which actually does not use the value of $\alpha_0$, can still work in this case and achieve an $\widetilde{O}(T^{2/3})$ regret. The regret lower bound also directly follows the third statement of \Cref{thm: known alpha unknown G} since any bidding strategy cannot obtain a better regret guarantee than $O(T^{2/3})$ when $\alpha_0 = 0$. Hence, we have the following result. 

\begin{corollary}
\label{cor: unknown alpha unknown G}
For repeated non-credible second-price auctions with unknown credibility $\alpha_0$, unknown distribution $G$ and bandit feedback, there exists a bidding algorithm (\Cref{algo: known alpha unknown G fpa}) that achieves an $\widetilde{O}(T^{2/3})$ regret, and the lower bound on regret for this problem is $\Omega(T^{2/3})$.
\end{corollary}

Despite the sublinear regret, the result of \Cref{cor: unknown alpha unknown G} is not satisfactory. \Cref{algo: known alpha unknown G fpa} only falls into the category of usual UCB policies with cross learning, but does not make full use of the properties of this auction setting. In fact, it treats the seller's mechanism as a black box without really estimating the seller's credibility or other bidder's strategies.

% The latter idea of designing a bidding algorithm, which solely focuses on selecting bids based on historical average rewards or the least number of explorations, neglects the crucial aspect of estimating the parameters in the seller's auction rules and the distribution of market competition bids. While it is true that the latter algorithm may achieve a higher total return than the former algorithm, it is important to consider the long-term business strategic significance and the limitations of this approach.

% By treating the seller and the market as a black box and disregarding parameter estimation, the algorithm fails to capture the underlying dynamics and intricacies of the auction environment. Without estimating the parameters, the algorithm lacks the ability to adapt to changes in the auction rules or the behavior of other bidders. This can lead to suboptimal bidding decisions and missed opportunities for maximizing rewards.

% Estimating the parameters in the seller's auction rules and the distribution of market competition bids is crucial for several reasons. Firstly, it allows for a deeper understanding of the auction dynamics, enabling the bidder to make more informed decisions. By analyzing historical data and estimating these parameters, the algorithm can uncover patterns, trends, and potential biases in the auction process. This knowledge can be leveraged to strategically adjust bidding strategies and gain a competitive advantage.

% Furthermore, estimating the parameters provides valuable insights into the market landscape and the behavior of other bidders. Understanding the distribution of competitive bids helps in identifying potential competitors' strategies, their willingness to pay, and their overall market position. This information is essential for formulating effective bidding strategies that can outperform competitors and secure higher rewards.

% In addition to immediate benefits, estimating parameters also has long-term business significance. It allows for continuous learning and improvement of the bidding algorithm over time. By updating and refining the estimators based on new data, the algorithm can adapt to changing market conditions, evolving auction rules, and the dynamic behavior of other bidders. This adaptability ensures that the bidding algorithm remains effective and competitive in the long run.

% In conclusion, while the latter algorithm may achieve a higher total return in the short term, it fails to consider the necessity and business significance of estimating the parameters in the seller's auction rules and the distribution of market competition bids. By neglecting parameter estimation, the algorithm overlooks valuable insights, adaptability, and strategic advantages that can be gained through a more comprehensive approach. Estimating these parameters is essential for making informed bidding decisions, understanding the market landscape, and ensuring long-term success in the online bidding problem.

% The latter idea of designing a bidding algorithm, which solely focuses on selecting bids based on historical average rewards or the least number of explorations, lacks a comprehensive understanding of the underlying auction dynamics. By treating the seller and the market as a black box, this approach overlooks the crucial aspect of estimating the unknown parameters in the seller's auction rules and the distribution of competitive bids.

% Estimating these parameters is of utmost importance as it provides valuable insights into the auction environment and allows for a more informed bidding strategy. Without estimating the parameters, the algorithm fails to capture the nuances and intricacies of the auction, potentially leading to suboptimal bidding decisions.

% Furthermore, estimating the parameters in the seller's auction rules and the distribution of market competition bids holds significant strategic significance. By gaining a deeper understanding of these parameters, bidders can uncover valuable information about their competitors' behavior and adjust their bidding strategies accordingly. This knowledge can provide a competitive advantage and potentially lead to higher rewards in the auction.

% In contrast, the latter algorithm's reliance solely on historical average rewards or the least number of explorations oversimplifies the complexity of the auction dynamics. It fails to adapt to changing market conditions or account for potential variations in bidding patterns over time. By neglecting the estimation of parameters, it misses out on the opportunity to optimize bidding decisions based on a more accurate understanding of the auction environment.

% In conclusion, the former idea of designing a bidding algorithm, which involves estimating the parameters in the seller's auction rules and the distribution of competitive bids based on historical data, is essential for developing a robust and effective bidding strategy. This approach enables bidders to make more informed decisions, adapt to market dynamics, and potentially outperform competitors in the repeated auction scenario.


\paragraph{Full feedback.} With the above in mind, we explore whether we can make any improvements with richer feedback and more meticulous estimation of $\alpha_0$ and $G$. In the full feedback model, $p_t = \alpha_0 d_t + (1-\alpha_0)b_t$ is always observable, which would intuitively help our estimation. Nevertheless, when $\alpha_0 = 0$, binary feedback in first-prices auctions still results in the $\Omega(T^{2/3})$ lower bound. Thus, in what follows we exclude the extreme case of $\alpha=0$ when it is impossible to achieves a better bound than $O(T^{2/3})$. Note that sellers in reality often do not set $\alpha_0 = 0$ due to concerns about reputation or cheating costs \cite{mcadams2007pays}. This assumption is also consistent with the recent empirical findings by \citet{dianat2021credibility} that although sellers in non-credible second-price auctions often overcharge, they typically do not use the rules of the first-price auction to maximize revenue.

\begin{assumption}
\label{asm: unknown alpha unknown G}
There exists a constant $\underline{\alpha} > 0$ such that $\alpha_0 \in [\underline{\alpha}, 1]$.
\end{assumption}

\begin{restatable}{theorem}{fourththeorem}
\label{thm: unknown alpha unknown G bandit}
Suppose that \Cref{asm: unknown alpha unknown G} holds. For repeated non-credible second-price auctions with unknown credibility $\alpha_0$, known distribution $G$ and bandit feedback, the lower bound on regret for this problem is $\Omega(T^{1/2})$. If \Cref{asm: unknown alpha known G} holds, then there exists a bidding algorithm (\Cref{algo: unknown alpha unknown G bandit}) that achieves an $\widetilde{O}(T^{1/2})$ regret.
\end{restatable}

\begin{algorithm}[t]
\caption{Learning with unknown $\alpha_0$, unknown $G$ and bandit feedback}
\label{algo: unknown alpha unknown G bandit}
    \SetKwInput{KwInit}{Initialization}
    \KwIn{Time horizon $T$}
    \KwInit{set fail probability $\delta \in (0, 1)$.}
    \For{$t=1, \cdots, T$}{
    Receive the value $v_t \in [0, 1]$.\\
    Estimate $\alpha_0$ by choosing $\widetilde{\alpha}_t$,
    \begin{align}
        \widetilde{\alpha}_t = \inf\{\alpha \in [\underline{\alpha}, 1] | \calL_t(\alpha) \leq 0\},
    \end{align}
    where $\calL_t(\alpha)$ is defined by 
    \begin{align}
    % \label{eqn: estimate L}
        \calL_t(\alpha) = \sum_{s=1}^{t-1}x_s\bbI\left\{c_s\leq (1-\alpha)b_s\right\}.
    \end{align}\\
    Estimate $G$ by using $\hat{G}_t(x;\widetilde{\alpha}_t)$, defined by
    \begin{align}
    \label{eqn: empirical G}
        \hat{G}_t(x;\alpha) = \frac{1}{t-1} \sum_{s=1}^{t-1}\bbI \left\{\hat{d}_s(\alpha) \leq x\right\},
    \end{align}
    where $\hat{d}_s(\alpha) = (p_s - (1-\widetilde{\alpha})b_s)/\alpha_t$.\\
    Submit a bid $b_t$, computed by,
    \begin{align}
        b_t = \argmax_{b\in [1/(1 + \log t), 1]} \Big[ & \left(v_t - b\right)\hat{G}_{t}(b) \nonumber \\
        + \widetilde{\alpha}_{t} & \int_{0}^{b}\hat{G}_{t}(y)\,dy \Big],
    \end{align}
    }
\end{algorithm}

The corresponding algorithm is presented in \Cref{algo: unknown alpha unknown G bandit}. In each round $t$, the bidder chooses the minimum value that can make the loss function $\calL_t(\alpha)$ zero as the estimate of $\alpha_0$. Observe that $\calL_t(\alpha)$ is an non-increasing function in $\alpha$. 
This can be done efficiently using binary search. Then given a good estimate $\widetilde{\alpha}_t$, $G$ can be approximated well by the empirical distribution $\hat{G}_t(;\widetilde{\alpha}_t)$ using samples
$\{\hat{d}_s(\widetilde{\alpha}_t)\}_{s=1}^{t-1}$. 
Finally, the bidder submits a $b_t$ that maximizes the estimated expected reward based on the estimated parameter $\widetilde{\alpha}_t$ and the estimated distribution $\hat{G}_t(;\widetilde{\alpha}_t)$. The following \Cref{lem: estimate G} is a key ingredient used to prove the result of \Cref{thm: unknown alpha unknown G bandit}.

\begin{lemma}
\label{lem: estimate G}
    Suppose that $G$ is $B_2$-Lipschitz. When $|\alpha - \alpha_0| \leq \calK$, we have probability at least $1-\delta$, $\forall x\in [0, 1]$,
    \begin{align*}
        |\hat{G}_t(x)- G(x)| \leq & B_2\calK /\alpha_0 +  \sqrt{\frac{\log(4/\delta)}{2(t-1)}}.
    \end{align*}
\end{lemma}

% \paragraph{Full feedback.} Now, we explore the full feedback model where $p_t = \alpha_0 d_t + (1-\alpha_0)b_t$ is always observable, which would intuitively help our estimation. 

% Nevertheless, when $\alpha_0 = 0$, binary feedback in first-prices auctions still results in the $\Omega(T^{2/3})$ lower bound. Thus, in what follows we exclude the extreme case of $\alpha=0$ when it is impossible to achieves a better bound than $O(T^{2/3})$. Note that sellers in reality often do not set $\alpha_0 = 0$ due to concerns about reputation or cheating costs \cite{mcadams2007pays}. This assumption is also consistent with the recent empirical findings by \citet{dianat2021credibility} that although sellers in non-credible second-price auctions often overcharge, they typically do not use the rules of the first-price auction to maximize revenue.

% We also make a mild assumption over $G$. 
% \begin{assumption}
% \label{asm: unknown alpha unknown G 2}
%     $G$ is $B_2$-Lipschitz, i.e., for $\forall x, x' \in \bbR$, we have $|G(x) - G(x')| \leq B_2|x - x'|$. 
% \end{assumption}

% Given that \Cref{asm: unknown alpha unknown G 2} holds, we show that $G$ can be approximated if we have a good estimate of $\alpha$. Let $\hat{d}_s(\alpha) = (p_s - (1 - \alpha)b_s)/\alpha$ be the inferred highest competing bid in round $s$ with $\alpha$, and let $\hat{G}_t(;\alpha)$ be the empirical distribution of samples $\{\hat{d}_s\}_{s=1}^{t-1}$, i.e.
% \begin{align}
% \label{eqn: empirical G}
%     \hat{G}_t(x;\alpha) = \frac{1}{t-1} \sum_{s=1}^{t-1}\bbI \left\{\hat{d}_s(\alpha) \leq x\right\}.
% \end{align}

% \begin{lemma}
% \label{lem: estimate G}
%     Suppose that \Cref{asm: unknown alpha unknown G 2} holds. When $|\alpha - \alpha_0| \leq \calK$, we have probability at least $1-\delta$, $\forall x\in [0, 1]$,
%     \begin{align*}
%         |\hat{G}_t(x)- G(x)| \leq & B_2\calK /\alpha_0 +  \sqrt{\frac{\log(4/\delta)}{2(t-1)}}.
%     \end{align*}
% \end{lemma}

\begin{algorithm}
\caption{Learning with unknown $\alpha_0$, unknown $G$ and full feedback}
\label{algo: unknown alpha unknown G full}
    \SetKwInput{KwInit}{Initialization}
    \KwIn{Time horizon $T$}
    \KwInit{Let $\calA = \{\alpha^1, \cdots, \alpha^M\}$ be the credibility set with $\alpha^m = m/M$; let $\calB = \{b^1, \cdots, b^K\}$ be the bid set with $b^k = k/K$; set learning rate $\eta > 0$ and fail probability $\delta \in (0, 1)$.}
    \For{$t=1, \cdots, T$}{
    Receive the value $v_t \in [0, 1]$.\\
    Sample a parameter $\alpha_t$ from $q_t$, a distribution over $\calA$ defined via $q_t \propto \exp{(-\eta \sum_{s=1}^{t-1} \hat{\ell}_{s, m})}$.\\
    Estimate the reward $\widetilde{r}_t(v_t, b^k, \alpha^m)$ for every $k \in [K]$ and every $m\in [M]$ by \eqref{eqn: empirical r}, and compute
    \begin{align*}
        b_{t, \alpha^{m}} \in \arg\max_{b\in \calB} \left( \widetilde{r}_t(v_t, b^k, \alpha_t) + w_t\right).
    \end{align*}
    where $w_t = \sqrt{2\log T/(t-1)}$.\\
    Submit $b_t = b_{t, \alpha_t}$ and observe $p_t$.\\
    Compute the loss $\hat{\ell}_{t, m}$ for every $m \in [M]$ by
    \begin{align}
        \hat{\ell}_{t, m} = \frac{\bbI \left[b_{t, \alpha^m} = b_t\right]}{P_t(b_{t})}(1 - r_t),
    \end{align}
    where $P(b) = \bbE_{\alpha \sim q_t}\left[\bbI\left\{b_{t, \alpha} = b\right\}\right]$.
    }
\end{algorithm}

Next, we introduce another algorithm, \Cref{algo: unknown alpha unknown G full}, which combines the ideas of \textbf{Exp3} \cite{auer2002nonstochastic} and \textbf{UCB1.CL} \cite{balseiro2019contextual}, which are classic algorithms for contextual multi-armed bandit problems.

We model each $\alpha^m$ in a discretized space $\calA = \{0, 1/M, 1/M, \cdots, 1\}$ as a predictor, who behaves as if $\alpha^m$ is the real credibility parameter. The idea of \textbf{Exp3} is to maintain a distribution $q_t$ over these experts and update it via a classical exponential
weight scheme: $q_t \propto \exp{(-\eta \sum_{s=1}^{t-1} \hat{\ell}_{s, m})}$ where $\hat{\ell}_{s, m}$ is an estimator for some loss $\ell_{s, m}$ of $\alpha^m$. In each round $t$, we sample an expert $\alpha_t$ from $q_t$ and submit $b_{t, \alpha_t}$ suggested by $\alpha_t$.

For each $\alpha^m$, we maintain a UCB estimate of the expected reward under each $b^k$, 
\begin{align}
    \widetilde{r}_t(v_t, b^k, \alpha^m) = & (v_t - b^k)\hat{G}_s(b^k;\alpha^m) \nonumber \\
    & + \alpha^m \int_{0}^{b^k} \hat{G}_s(x;\alpha^m) dx, \label{eqn: empirical r}
\end{align}
where $\hat{G}_s(;\alpha^m)$ is the empirical distribution defined as in \eqref{eqn: empirical G}.
If $m$-th predictor is selected, it submits the bid with the highest UCB estimate. Note that if the $m$-th predictor believes $\alpha^m = \alpha_0$, it also believes the property of cross-learning over values and actions should hold under full feedback , i.e., given $r_t$ under $(v_t, b_t)$, it can compute $r'$ under any other $(v', b')$ since it can recover the ``true'' $d_t$. Wrong beliefs lead some predictors to use inaccurate UCB estimates and submit some outrageous bids, but we downweight them precisely because following their suggestion would result in too low rewards.

\begin{restatable}{theorem}{thirdtheorem}
\label{thm: unknown alpha unknown G full}
Suppose that \Cref{asm: unknown alpha unknown G} holds. For repeated non-credible second-price auctions with unknown credibility $\alpha_0$, known distribution $G$ and full feedback, the lower bound on regret for this problem is $\Omega(T^{1/2})$. If $G$ is Lipschitz continuous, there exists a bidding algorithm (\Cref{algo: unknown alpha unknown G full}) that achieves $\widetilde{O}(T^{2/3})$.
\end{restatable}

We prove \Cref{thm: unknown alpha unknown G full} in two steps. First, we bound the relative loss of \Cref{algo: unknown alpha unknown G full} compared with any single predictor in terms of the expected total reward. Next, with \Cref{lem: estimate G} in hand, it is straightforward to show that if $\alpha_m$ is close to $\alpha_0$, the loss incurred by the strategy that always follows the suggestion of the $m$-th predictor is small. Finally, putting everything together and setting $K \sim T^{1/3}, \delta \sim T$ and $\eta \sim T^{2/3}$, we obtain the $\widetilde{O}(T^{2/3})$ regret bound.

Despite the worse regret bound of \Cref{algo: unknown alpha unknown G full} compared with \Cref{algo: unknown alpha unknown G bandit}. It only requires Lipschitz continuity over distribution $G$, while the regret guarantee \Cref{algo: unknown alpha unknown G bandit} relies heavily on the density lower bound. Since we use an EXP policy to choose $\alpha_t$ and a UCB policy to choose $b_t$, one may wonder whether we are able to make them consistent. We conjecture it is possible to replace the latter UCB with EXP, and then the algorithm can potentially handle adversarial competing bids, which we leave as an open problem. However, the strategy path under a fix $\alpha^m$ is hard to track, so unfortunately we fail to give a UCB estimate of some statistic under each $\alpha^m$. It may require more techniques and efforts to apply a UCB policy to choose $\alpha_t$.

Since $p_s$ is observable at each round in the full feedback model, one may consider to view it as a linear regression problem $p_s = \beta_1 b_s + \beta_0 + \epsilon_s$ where $\beta_1 = (1-\alpha_0), \beta_0 = \alpha_0\bbE \left[d_s\right]$ and $\epsilon_s = \alpha_0(d_s - \bbE \left[d_s\right])$. Then the estimated coefficient $\hat{\beta}_{1, t}$, combined with \Cref{lem: estimate G}, appears promising for calculating a good bid $b_t$. However, the convergence rate of $\hat{\beta}_{1, t}$ depends on the variance of independent variables, i.e., the historical bids, which we cannot fully control in some bad cases. For example, when $v_t \equiv 1$, it requires $b_t \rightarrow b^*(1, \alpha_0)$ for an algorithm to achieve lower regret. But when all historical bids are approaching $b^*(1, \alpha_0)$, the variance can be undesirable.
